On Optimization Modulo Theories, MaxSMT and Sorting Networks

Optimization Modulo Theories (OMT) is an extension of SMT which allows for finding models that optimize given objectives. (Partial weighted) MaxSMT --or equivalently OMT with Pseudo-Boolean objective functions, OMT+PB-- is a very-relevant strict subcase of OMT. We classify existing approaches for MaxSMT or OMT+PB in two groups: MaxSAT-based approaches exploit the efficiency of state-of-the-art MAXSAT solvers, but they are specific-purpose and not always applicable; OMT-based approaches are general-purpose, but they suffer from intrinsic inefficiencies on MaxSMT/OMT+PB problems. We identify a major source of such inefficiencies, and we address it by enhancing OMT by means of bidirectional sorting networks. We implemented this idea on top of the OptiMathSAT OMT solver. We run an extensive empirical evaluation on a variety of problems, comparing MaxSAT-based and OMT-based techniques, with and without sorting networks, implemented on top of OptiMathSAT and {\nu}Z. The results support the effectiveness of this idea, and provide interesting insights about the different approaches.

==> abstract.tex.1 <==
\noi
Optimization Modulo Theories (\omt) is an extension of \smt which
allows for finding models that make given
objectives optimum.
%
% \ignore{
% \omt has been extended to be incremental and to handle multiple
% objective functions either independently or with their linear,
% lexicographic, Pareto, \minmax/\maxmin combinations.
% }
%
\omt applications can be found not only \ignoreinshort{in the domain of} Formal
Verification and related domains, 
\ignoreinshort{Automated 
Reasoning and Planning with Resources,} but also in other disciplines
like Machine Learning and
Requirement Engineering. \\ %\newline
%
(Partial weighted) \maxsmt --or, alternatively, \omt with
Pseudo-Boolean objective functions-- is a very-relevant subcase of
\omt. On the one hand, specialized approaches based on \maxsat solvers
may be very efficient for these problems, but they are not always applicable. 
On the other hand, \omt-based algorithms for \maxsmt suffer
from some intrinsic inefficiencies in some cases.  In this paper we
identify the sources of such inefficiencies and address them by
enhancing general \omt by means of sorting networks. We implemented
this idea on top of the \optimathsat \omt solver and evaluated them
empirically on problems coming from Machine Learning and
Requirement Engineering.
%
The empirical results support the effectiveness of this idea.


==> combining.tex.1 <==
A solution for improving search efficiency when dealing with \maxsmt 
and \omt with Pseudo-Boolean objectives in the form
\begin{eqnarray}
\label{eq:obj}
  \cost = w \cdot \sum_{i=0}^{i=n-1} A_i
\end{eqnarray}
\noi
is to reduce the dependency on the expensive \laratsolver{} by better 
exploiting Boolean Constraint Propagation (BCP) with the aid of 
sorting networks.

A sorting-network relation, depicted in figure \ref{fig:snetwork}, 
takes $A_0, ..., A_{n-1}$ Boolean variables as input
and returns $out_0, ..., out_{n-1}$ variables as output s.t., if 
in the current (partial) truth assignment $\mu$, $k$ variables are set to True, 
$n-m$ variables are set to False and $m-k$ are unassigned,
then by Boolean Constraint Propagation $out_0, ..., out_{k-1}$ are set to True, 
$out_m, ..., out_{n-1}$ are set to False and
$out_k, ..., out_{m-1}$ are not propagated. 
%
%\RSTODO{Il punto del messaggio  ``sort'' ==  $F < \star < \top$ mi e' poco chiaro}

For our purposes, it is important that the implementation of the
relation is {\em bidirectional}: e.g., if $out_{k-1}$ is forced to be
True (that is, at least $k$ inputs must be True) and $n-k$ inputs
$A_i$ are False, then by Boolean Propagation all other unassigned
$A_i$s are automatically set to True; vice-versa, if $out_{k+1}$ is
forced to be False (that is, at most $k$ inputs can be True) and $n-k$
inputs $A_i$ are True, then all other unassigned $A_i$s
 are automatically set to False.

\begin{figure}[tb]
\centering
\includegraphics[scale=0.3]{png/circuit1.png}
\caption{\label{fig:snetwork} The basic schema of a sorting network relation }
\end{figure}

Given an \omt problem $\langle \varphi , \cost , \rangle$, where 
$\cost$ is as in \eqref{eq:obj}, and a
sorting network relation encoding $C$ matching the previous definition,
we extend $\varphi$ in equation \eqref{eq:maxsmt2} as follows: 

\begin{equation}\label{eq:circuitb}
\varphi' = \varphi \wedge C \wedge \bigwedge_{k=0}^{k=n-1} 
\begin{cases}
out_{k} \rightarrow ((k+1)\cdot w \leq \cost) \\
\neg out_{k} \rightarrow (\cost \leq k \cdot w) \\
\neg((k+1)\cdot w \leq \cost) \vee \neg(\cost \leq k \cdot w)
\end{cases}
\end{equation}
\noi
and optimize $\cost$ over $\varphi'$.
%
Notice here that the third line in equation \ref{eq:circuitb} is \T-valid, but it allows for
assigning the value of some variables $out_i$ by BCP as soon as a unit clause
in the form $(\cost \leq k \cdot w)$ is added to the formula.

The benefit of this extension is that now, whenever the optimization
search finds a new satisfiable truth assignment $\mu$ which sets $k$
variables $A_i$ to True, so that a unit clause in the form $(\cost < k\cdot
w)$ is learned, then as soon as $k-1$ inputs $A_i$ are assigned to True
the remaining $n-k+1$ 
inputs are set to False by BCP.
(A dual case occurs when some lower-bound unit clause $(\cost > k\cdot
w)$ is learned.)

In our work, we have considered two encodings for the sorting network relation: 
the sequential counter encoding \cite{Sinz05} 
and the cardinality network encoding \cite{parametricCardinalityConstraint}. 
%
<<<<<<< .mine

%\PTNOTE{
=======
>>>>>>> .r50
Notice that, in contrast with the literature which usually focuses on only one direction
of cardinality constraints, in our context we are interested in a bidirectional encoding
of sorting circuit so to ensure the correct propagation of the $out_k$ values. 
<<<<<<< .mine
This is due to the fact that our \omt solver can apply this technique
not only to deal with Pseudo-Boolean objectives that can either be minimized or maximized,
but also with generic Pseudo-Boolean sums subject to some cardinality constraints outside
of an optimization context.
%}
=======
This is due to the fact that our \omt solver applies this technique
to deal not only with MaxSMT problems but also with Pseudo-Boolean objectives that can 
be either minimized or maximized, and other Pseudo-Boolean sums subject to simple 
cardinality constraints outside of an optimization context.
>>>>>>> .r50

\subsubsection*{Bidirectional Sequential Counter Encoding}

The sequential counter encoding $LT_{SEQ}^{n,k}$ for $\leq k (A_0, ..., A_{n-1})$ presented in \cite{Sinz05} requires 
$O(k\cdot n)$ clauses and variables to be represented, and is arc-consistent. 
The circuit is given by the composition of $n$ sub-circuits, each of which
computes $s_i = \sum_{j=0}^{j=i}A_j$, represented in unary form with the bits $s_{i, j}$. The following formula is the original propositional 
encoding of $LT_{SEQ}^{n,k}$ presented in \cite{Sinz05}, with $k$ instantiated to $n$, which was obtained after discarding one 
direction of the equations for polarity reasons. 
\[
\begin{array}{l}
(\neg A_{0}\vee s_{0,0}) \wedge
\bigwedge_{i=1}^{i=n-1}
	\{
	(\neg A_{i}\vee s_{i,0}) \wedge
	(\neg s_{i-1,0}\vee s_{i,0}) \wedge
	(\neg A_{i}\vee\neg s_{i-1,n}) \wedge
	\} \\
\bigwedge_{j=1}^{j=n-1} \{
	(\neg s_{0,j}) \} \wedge
\bigwedge_{i,j=1}^{i,j=n-1} \{
	(\neg A_{i}\vee\neg s_{i-1,j-1}\vee s_{i,j}) \wedge
	(\neg s_{i-1,j}\vee s_{i,j}) \}
\end{array}	
\]
%
%For our own application, we need both directions of the equations to ensure 
%that  the $out_k$ values are correctly propagated even when the 
%circuit is subject to maximization constraints or no constraint at all.
%
%Thus, we strengthened the formula given in \cite{Sinz05} with the following clauses:
We strengthened the original encoding with the following clauses to make it bidirectional:
\[
\begin{array}{l}
(A_{0}\vee\neg s_{0,0}) \wedge

\bigwedge_{i=1}^{i=n-1}
\{
	(\neg s_{i,0}\vee A_{i}\vee s_{i-1,0})
\} \wedge
\bigwedge_{i,j=1}^{i,j=n-1}
(\neg s_{i,j}\vee s_{i-1,j}\vee(s_{i-1,j-1}\wedge A_{i}))
\end{array}
\]

\ignore{ % deprecated formula
\[
\begin{array}{l}
(A_{0}\vee\neg s_{0,0})\\
\begin{rcases*}
(\neg s_{i,0}\vee A_{i}\vee s_{i-1,0})\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\\
\end{rcases*}
i \in [1,n[ \\
\begin{rcases*}
(\neg s_{i,j}\vee s_{i-1,j}\vee(s_{i-1,j-1}\wedge A_{i}))\:\:\:\:\:\\
\end{rcases*} 
j \in [1,n[ \: \wedge \: i \in [1,n[ \\
\end{array}
\]
}

\subsubsection*{Bidirectional Cardinality Network Encoding}

The cardinality network encoding presented in \cite{EenS06,Asin2011,parametricCardinalityConstraint},
based on the underlying sorting scheme of the well-known \textit{merge-sort} algorithm,
has complexity $O(n \log^2 k)$ in the number of clauses and variables, and is arc-consistent. 
%
Due to space limitations, we refer the reader to \cite{parametricCardinalityConstraint} for the
encoding of cardinality networks we used in our own work. Notice that, differently than in the
previous case, this sorting circuit propagates values in both directions and is thus suitable
to be used as is within \omt.

%If we consider that for our purposes $k = n$, since we generate the circuit prior to starting
%the search, then it is clear that the encoding presented in \cite{parametricCardinalityConstraint}
%looks more appealing than the sequential counter encoding due to its lower complexity 
%in terms of clauses and variables needed.


\ignore{
For example, instead of learning the unit clause $(\cost \leq ub)$ at each satisfiable step of the 
minimization search, a possible approach is to learn $(\cost \leq k\cdot w) \wedge \leq 
k (A_0, ..., A_{n-1})$, where $\leq k (A_0, ..., A_{n-1})$ is a Boolean formula forcing 
at most $k$ out of the $n$ variables $A_0, ..., A_{n-1}$  to be assigned True and 
$ub = k \cdot w$. Dual for maximization.

As a result, the Boolean engine no longer needs the \laratsolver{} in order to prune those 
(partial) truth assignments $\mu'$ that would not improve over the current value of $\cost$.

This approach has some limitations:
\begin{itemize}
\item if the input problem is unsatisfiable, then the formula encoding the cardinality constraint $\leq k (A_0, ..., A_{n-1})$ is 
never learned and as a result there is no performance improvement
\item if the objective function is the result of a non-trivial combination of multiple terms, including Pseudo-Boolean terms,
the value $k$ to be used in the cardinality constraint $\leq k (A_0, ..., A_{n-1})$ is of non-trivial computation
\item any Pseudo-Boolean term appearing as part of equality or inequality constraints and not
included in the definition of some objective function does not benefit from the solution \PTNOTE{move afterwards as bonus}
\end{itemize}

In order to overcome these issues a better solution is to assume, for each objective $\cost \triangleq w\cdot\sum_i A_i$ 
that needs to be minimized, the following formula 
\begin{equation}\label{eq:circuita}
\bigwedge_{k=0}^{k=n-1} (\cost \leq k\cdot w) \leftrightarrow \leq k (A_1, ..., A_n)
\end{equation}
at the beginning of the search.
}


==> combining.tex.2 <==
\begin{figure}[tb]
\centering
\includegraphics[scale=0.36]{png/circuit1.png}
\caption{\label{fig:snetwork} The basic schema of a sorting network relation. }
\end{figure}

A solution for improving search efficiency when dealing with \maxsmt 
and \omt with Pseudo-Boolean objectives in the form
\begin{eqnarray}
\label{eq:obj}
\textstyle
  \cost = w \cdot \sum_{i=0}^{n-1} A_i
\end{eqnarray}
\noi
is to reduce the dependency on the expensive \laratsolver{} by better 
exploiting Boolean Constraint Propagation (BCP) with the aid of Boolean
{\em sorting networks}.

A Boolean sorting-network relation 
${\sf  SN}(\underline{A},\underline{out})$, 
depicted in Figure~\ref{fig:snetwork},
between $n$ Boolean variables $\underline{A}\defas\set{A_0, ...,
  A_{n-1}}$ and $n$ Boolean variables $\underline{out}\defas
\set{out_0, ..., out_{n-1}}$, is described as follows: 
%maintains the following invariant, 
in every partial 
truth assignment $\mu$ which satisfies {\sf  SN}(\underline{A},\underline{out}),
%
\begin{equation}
\label{eq:sorting-network}
\left \{
\begin{tabular}{rl}
$k$ variables in \underline{A}    &are $\top$,\\
$n-m$ variables in \underline{A}  &are $\bot$,\\
$m-k$ variables  in \underline{A} &are $*$,\\
\end{tabular}
\right \}
%\Longleftrightarrow
\mbox{if and only if}
%\mbox{iff}
\left \{
\begin{tabular}{ll}
$out_0, ..., out_{k-1}$ &are $\top$,\\
$out_m, ..., out_{n-1}$ &are $\bot$,\\
$out_k, ..., out_{m-1}$ &are $*$.\\
\end{tabular}
\right \}  
\end{equation}
\noi
for every $m,k$ s.t. $n\ge m \ge k \ge 0$.


Intuitively, $\underline{out}$ is a sorted version of
\underline{A} according to the ordering 
``$\top < * < \bot$'', so that $out_i$ is $\top$ iff 
at least $i+1$ variables in \underline{A} are $\top$, 
it is $\bot$ iff at least $n-i$ such variables are $\bot$.  
~%
%\footnote{
Notice that, 
for every $i$, 
if $out_i$ is $\top$, 
then also $out_0,...,out_{i-1}$ must be $\top$, and that 
if $out_i$ is $\bot$, 
then also $out_{i+1},...,out_{n-1}$ must be $\bot$.
% }

%\RSTODO{spiega bene, spiega anche in avanti, e il caso di conflitto}

For our purposes, it is important that the implementation 
of ${\sf  SN}(\underline{A},\underline{out})$ maintains the
sorting-network relation \eqref{eq:sorting-network} by
BCP, in a  {\em bi-directional} way: 
any partial assignment $\mu_0$ which does not verify {\em
  bi-directional} either is extended by BCP to one which verifies it, or a
conflict is produced if no such extension exists. 
%
For instance:
%
\begin{itemize}
\item 
if (exactly) $k$ variables in \underline{A} are $\top$ and $n-m$
  are $\bot$, then $out_0, ..., out_{k-1}$ are set $\top$ and 
$out_m, ..., out_{n-1}$ are set $\bot$ by BCP (if unassigned);
\item 
if $out_{i}$ is 
$\top$, then $out_{0},...,out_{i-1}$ are also set to $\top$
by BCP (if unassigned);
\item 
if $out_{i}$ is 
$\bot$, then $out_{i+1},...,out_{n-1}$ are also set to $\top$
by BCP (if unassigned);
\item if $out_{k-1}$ is $\top$ and $n-k$ variables in \underline{A} 
$A_i$ are  $\bot$, then by BCP all other unassigned
$A_i$s are automatically set to $\top$; 
\item if $out_{k+1}$ is $\bot$ and $n-k$ variables in \underline{A} 
$A_i$ are  $\top$, then by BCP all other unassigned
$A_i$s are automatically set to $\bot$;
\end{itemize}
If any of the above BCP assignments conflicts with some previous
assignments, a conflict is produced. 

% vice-versa, if $out_{k+1}$ is
% forced to be False (that is, at most $k$ inputs can be True) and $n-k$
% inputs $A_i$ are True, then all other unassigned $A_i$s
%  are automatically set to False.


Given an \omt problem $\langle \varphi , \cost , \rangle$, where 
$\cost$ is as in \eqref{eq:obj}, and a Boolean formula ${\sf
  SN}(\underline{A},\underline{out})$ encoding a sorting network
relation which matches the previous definition,
we extend $\varphi$ in \eqref{eq:maxsmt2}-\eqref{eq:maxsmt3} as follows: 
%
\begin{equation}
\label{eq:circuitb}
\varphi' = \varphi \wedge {\sf SN}(\underline{A},\underline{out})
 \wedge \bigwedge_{k=0}^{k=n-1} 
\begin{cases}
out_{k} \rightarrow ((k+1)\cdot w \leq \cost) \\
\neg out_{k} \rightarrow (\cost \leq k \cdot w) \\
\neg((k+1)\cdot w \leq \cost) \vee \neg(\cost \leq k \cdot w)
\end{cases}
\end{equation}
\noi
and optimize $\cost$ over $\varphi'$.
%
Notice here that the third line in equation \ref{eq:circuitb} is \T-valid, but it allows for
assigning the value of some variables $out_i$ by BCP as soon as a unit clause
in the form $(\cost \leq k \cdot w)$ is added to the formula.

The benefit of this extension is that now, whenever the optimization
search finds a new satisfiable truth assignment $\mu$ which sets $k$
variables $A_i$ to True, so that a unit clause in the form $\neg(k\cdot
w \leq \cost)$ is learned, then as soon as $k-1$ inputs $A_i$ are assigned to True
the remaining $n-k+1$ 
inputs are set to False by BCP.
(A dual case occurs when some lower-bound unit clause $\neg(\cost \leq k\cdot
w)$ is learned.)

\newpage
\begin{figure}[tb]
	\begin{center}
		\includegraphics[scale=0.38]{png/solution_01.png}\\
	\end{center}
\caption{\label{fig:sol1}
\textmd{An example of \omt search with sorting networks.
}}
\end{figure}
%
%{\subsubsection*{Example (continued).} 

  \begin{example}
\label{ex:withcardinalitynetwork}
Consider Example~\ref{ex:nocardinalitynetwork}.
  Figure~\ref{fig:sol1}
  shows the same example in which we extend the encoding with the
  sorting-network relation as in \eqref{eq:circuitb}. 
  The behaviour is identical to that of
  Example~\ref{ex:nocardinalitynetwork}
  until the assignment $\mu_1$ is generated, the unit clause $\neg(2
  \leq \cost)$ is learned, and the procedure backtracks for the first
  time (Figure~\ref{fig:sol1} left). 

As soon as $A_0$ is picked as new
  decision, the conjunction of the $\neg(2 \leq \cost)$ and the
  sorting-network relation causes the immediate BCP of the values
  $\neg A_1$, $\neg A_2$ and $\neg A_3$, without the need of multiple
  invocations of the (expensive) \laratsolver{}.    
\hfill $\diamond$  
\end{example}

In our work, we have considered two encodings for the sorting network relation: 
the sequential counter encoding \cite{Sinz05} 
and the cardinality network encoding \cite{parametricCardinalityConstraint}. 
%
Notice that, in contrast with the literature which usually focuses on
only one direction of cardinality constraints, in our context we are
interested in a bidirectional encoding of sorting circuit so that to
ensure the correct propagation of the $out_k$ values.  This is due to
the fact that our \omt solver applies this technique to deal not only
with MaxSMT problems but also with Pseudo-Boolean objectives that can
be either minimized or maximized, and other Pseudo-Boolean sums
subject to simple cardinality constraints outside of an optimization
context.

\subsubsection*{Bidirectional Sequential Counter Encoding}

The sequential counter encoding $LT_{SEQ}^{n,k}$ for $\leq k (A_0, ..., A_{n-1})$ presented in \cite{Sinz05} requires 
$O(k\cdot n)$ clauses and variables to be represented, and is arc-consistent. 
The circuit is given by the composition of $n$ sub-circuits, each of which
computes $s_i = \sum_{j=0}^{j=i}A_j$, represented in unary form with the bits $s_{i, j}$. The following formula is the original propositional 
encoding of $LT_{SEQ}^{n,k}$ presented in \cite{Sinz05}, with $k$ instantiated to $n$, which was obtained after discarding one 
direction of the equations for polarity reasons. 
\[
\begin{array}{l}
(\neg A_{0}\vee s_{0,0}) \wedge
\bigwedge_{i=1}^{i=n-1}
	\{
	(\neg A_{i}\vee s_{i,0}) \wedge
	(\neg s_{i-1,0}\vee s_{i,0}) \wedge
	(\neg A_{i}\vee\neg s_{i-1,n}) \wedge
	\} \\
\bigwedge_{j=1}^{j=n-1} \{
	(\neg s_{0,j}) \} \wedge
\bigwedge_{i,j=1}^{i,j=n-1} \{
	(\neg A_{i}\vee\neg s_{i-1,j-1}\vee s_{i,j}) \wedge
	(\neg s_{i-1,j}\vee s_{i,j}) \}
\end{array}	
\]
%
%For our own application, we need both directions of the equations to ensure 
%that  the $out_k$ values are correctly propagated even when the 
%circuit is subject to maximization constraints or no constraint at all.
%
%Thus, we strengthened the formula given in \cite{Sinz05} with the following clauses:
We strengthened the original encoding with the following clauses to make it bidirectional:
\[
\begin{array}{l}
(A_{0}\vee\neg s_{0,0}) \wedge

\bigwedge_{i=1}^{i=n-1}
\{
	(\neg s_{i,0}\vee A_{i}\vee s_{i-1,0})
\} \wedge
\bigwedge_{i,j=1}^{i,j=n-1}
(\neg s_{i,j}\vee s_{i-1,j}\vee(s_{i-1,j-1}\wedge A_{i}))
\end{array}
\]

\ignore{ % deprecated formula
\[
\begin{array}{l}
(A_{0}\vee\neg s_{0,0})\\
\begin{rcases*}
(\neg s_{i,0}\vee A_{i}\vee s_{i-1,0})\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\:\\
\end{rcases*}
i \in [1,n[ \\
\begin{rcases*}
(\neg s_{i,j}\vee s_{i-1,j}\vee(s_{i-1,j-1}\wedge A_{i}))\:\:\:\:\:\\
\end{rcases*} 
j \in [1,n[ \: \wedge \: i \in [1,n[ \\
\end{array}
\]
}

\subsubsection*{Bidirectional Cardinality Network Encoding}

The cardinality network encoding presented in \cite{EenS06,Asin2011,parametricCardinalityConstraint},
based on the underlying sorting scheme of the well-known \textit{merge-sort} algorithm,
has complexity $O(n \log^2 k)$ in the number of clauses and variables, and is arc-consistent. 
%
Due to space limitations, we refer the reader to \cite{parametricCardinalityConstraint} for the
encoding of cardinality networks we used in our own work. Notice that, differently than in the
previous case, this sorting circuit propagates values in both directions and is thus suitable
to be used as is within \omt.

%If we consider that for our purposes $k = n$, since we generate the circuit prior to starting
%the search, then it is clear that the encoding presented in \cite{parametricCardinalityConstraint}
%looks more appealing than the sequential counter encoding due to its lower complexity 
%in terms of clauses and variables needed.


\ignore{
For example, instead of learning the unit clause $(\cost \leq ub)$ at each satisfiable step of the 
minimization search, a possible approach is to learn $(\cost \leq k\cdot w) \wedge \leq 
k (A_0, ..., A_{n-1})$, where $\leq k (A_0, ..., A_{n-1})$ is a Boolean formula forcing 
at most $k$ out of the $n$ variables $A_0, ..., A_{n-1}$  to be assigned True and 
$ub = k \cdot w$. Dual for maximization.

As a result, the Boolean engine no longer needs the \laratsolver{} in order to prune those 
(partial) truth assignments $\mu'$ that would not improve over the current value of $\cost$.

This approach has some limitations:
\begin{itemize}
\item if the input problem is unsatisfiable, then the formula encoding the cardinality constraint $\leq k (A_0, ..., A_{n-1})$ is 
never learned and as a result there is no performance improvement
\item if the objective function is the result of a non-trivial combination of multiple terms, including Pseudo-Boolean terms,
the value $k$ to be used in the cardinality constraint $\leq k (A_0, ..., A_{n-1})$ is of non-trivial computation
\item any Pseudo-Boolean term appearing as part of equality or inequality constraints and not
included in the definition of some objective function does not benefit from the solution \PTNOTE{move afterwards as bonus}
\end{itemize}

In order to overcome these issues a better solution is to assume, for each objective $\cost \triangleq w\cdot\sum_i A_i$ 
that needs to be minimized, the following formula 
\begin{equation}\label{eq:circuita}
\bigwedge_{k=0}^{k=n-1} (\cost \leq k\cdot w) \leftrightarrow \leq k (A_1, ..., A_n)
\end{equation}
at the beginning of the search.
}

